Proceedings of the Workshop on Monte Carlo's, Physics and Simulations at the LHC PART I

These proceedings collect the presentations given at the first three meetings of the INFN "Workshop on Monte Carlo's, Physics and Simulations at the LHC", held at the Frascati National Laboratories in 2006. The first part of these proceedings contains pedagogical introductions to several basic topics of both theoretical and experimental high pT LHC physics. The second part collects more specialised presentations.

==> debug_log_27047 <==

#####Mon Feb  2 09:48:37 2009#####
STARTED admin_hep-ph.paolonason.2268


#####Mon Feb  2 09:48:37 2009#####
------------------------------------------------------------------------------
\\
arXiv:0902.0293
From: Paolo Nason <paolo.nason@mib.infn.it>
Date: Mon, 2 Feb 2009 13:38:47 GMT   (000kb)

Title: Proceedings of the Workshop on Monte Carlo's, Physics and Simulations at
  the LHC PART I
Authors: F. Ambroglini, R. Armillis, P. Azzi, G. Bagliesi, A. Ballestrero, G.
  Balossini, A. Banfi, P. Bartalini, D. Benedetti, G. Bevilacqua, S. Bolognesi,
  A. Cafarella, C.M. Carloni Calame, L. Carminati, M. Cobal, G. Corcella, C.
  Coriano', A. Dainese, V. Del Duca, F. Fabbri, M. Fabbrichesi, L. Fano', Alon
  E. Faraggi, S. Frixione, L. Garbini, A. Giammanco, M. Guzzi, N. Irges, E.
  Maina, C. Mariotti, G. Masetti, B. Mele, E. Migliore, G. Montagna, M.
  Monteno, M. Moretti, P. Nason, O. Nicrosini, A. Nisati, A. Perrotta, F.
  Piccinini, G. Polesello, D. Rebuzzi, A. Rizzi, S. Rolli, C. Roda, S. Rosati,
  A. Santocchia, D. Stocco, F. Tartarelli, R. Tenchini, A. Tonero, M. Treccani,
  D. Treleani, A. Tricoli, D. Trocino, L. Vecchi, A. Vicini, I. Vivarelli
Categories: hep-ph
Comments: 239 pages, 222 figures
License: http://arxiv.org/licenses/nonexclusive-distrib/1.0/
Policy: accept
Upload-archive: hep-ph
Upload-subject: hput admin_hep-ph.paolonason.2268
archive: hep-ph
is-an-author: 1
\\
  These proceedings collect the presentations given at the first three meetings
of the INFN "Workshop on Monte Carlo's, Physics and Simulations at the LHC",
held at the Frascati National Laboratories in 2006. The first part of these
proceedings contains pedagogical introductions to several basic topics of both
theoretical and experimental high pT LHC physics. The second part collects more
specialised presentations.
\\


#warnings_now: ADMIN UPLOAD



#author_warnings_now: 
Author 1: F. Ambroglini
Author 2: R. Armillis
Author 3: P. Azzi
Author 4: G. Bagliesi
Author 5: A. Ballestrero
Author 6: G. Balossini
Author 7: A. Banfi
Author 8: P. Bartalini
Author 9: D. Benedetti
Author 10: G. Bevilacqua
Author 11: S. Bolognesi
Author 12: A. Cafarella
Author 13: C.M. Carloni Calame
Author 14: L. Carminati
Author 15: M. Cobal
Author 16: G. Corcella
Author 17: C. Coriano'
Author 18: A. Dainese
Author 19: V. Del Duca
Author 20: F. Fabbri
Author 21: M. Fabbrichesi
Author 22: L. Fano'
Author 23: Alon E. Faraggi
Author 24: S. Frixione
Author 25: L. Garbini
Author 26: A. Giammanco
Author 27: M. Guzzi
Author 28: N. Irges
Author 29: E. Maina
Author 30: C. Mariotti
Author 31: G. Masetti
Author 32: B. Mele
Author 33: E. Migliore
Author 34: G. Montagna
Author 35: M. Monteno
Author 36: M. Moretti
Author 37: P. Nason
Author 38: O. Nicrosini
Author 39: A. Nisati
Author 40: A. Perrotta
Author 41: F. Piccinini
Author 42: G. Polesello
Author 43: D. Rebuzzi
Author 44: A. Rizzi
Author 45: S. Rolli
Author 46: C. Roda
Author 47: S. Rosati
Author 48: A. Santocchia
Author 49: D. Stocco
Author 50: F. Tartarelli
Author 51: R. Tenchini
Author 52: A. Tonero
Author 53: M. Treccani
Author 54: D. Treleani
Author 55: A. Tricoli
Author 56: D. Trocino
Author 57: L. Vecchi
Author 58: A. Vicini
Author 59: I. Vivarelli
-> Number of authors = 59



#####Mon Feb  2 09:48:39 2009#####
Finished unpacking (errors=)

#author_warnings_now: 
Author 1: F. Ambroglini
Author 2: R. Armillis
Author 3: P. Azzi
Author 4: G. Bagliesi
Author 5: A. Ballestrero
Author 6: G. Balossini
Author 7: A. Banfi
Author 8: P. Bartalini
Author 9: D. Benedetti
Author 10: G. Bevilacqua
Author 11: S. Bolognesi
Author 12: A. Cafarella
Author 13: C.M. Carloni Calame
Author 14: L. Carminati
Author 15: M. Cobal
Author 16: G. Corcella
Author 17: C. Coriano'
Author 18: A. Dainese
Author 19: V. Del Duca
Author 20: F. Fabbri
Author 21: M. Fabbrichesi
Author 22: L. Fano'
Author 23: Alon E. Faraggi
Author 24: S. Frixione
Author 25: L. Garbini
Author 26: A. Giammanco
Author 27: M. Guzzi
Author 28: N. Irges
Author 29: E. Maina
Author 30: C. Mariotti
Author 31: G. Masetti
Author 32: B. Mele
Author 33: E. Migliore
Author 34: G. Montagna
Author 35: M. Monteno
Author 36: M. Moretti
Author 37: P. Nason
Author 38: O. Nicrosini
Author 39: A. Nisati
Author 40: A. Perrotta
Author 41: F. Piccinini
Author 42: G. Polesello
Author 43: D. Rebuzzi
Author 44: A. Rizzi
Author 45: S. Rolli
Author 46: C. Roda
Author 47: S. Rosati
Author 48: A. Santocchia
Author 49: D. Stocco
Author 50: F. Tartarelli
Author 51: R. Tenchini
Author 52: A. Tonero
Author 53: M. Treccani
Author 54: D. Treleani
Author 55: A. Tricoli
Author 56: D. Trocino
Author 57: L. Vecchi
Author 58: A. Vicini
Author 59: I. Vivarelli
-> Number of authors = 59

 hep-ph.paolonason.2268.tar: unpacked 235 files from tar file


#####Mon Feb  2 09:48:39 2009#####
showtime: 0902.0293 being processed as test/9999151 -> /data/ftp/arxiv/papers/0902


#####Mon Feb  2 09:48:39 2009#####
packing to 0902.0293.tar.gz

#####Mon Feb  2 09:48:40 2009#####
running AutoTeX -p test/9999151 -d 0902.0293 at Mon Feb  2 09:48:40 2009

#####Mon Feb  2 09:48:44 2009#####
completed AutoTeX in 4s

#####Mon Feb  2 09:48:44 2009#####
Rejected after unpack_submission()... cleaning up

#warnings_now: ADMIN UPLOAD

Mon Feb  2 09:48:44 2009: AutoTeX took 4s


#####Mon Feb  2 09:48:44 2009#####
About to close and move this log to /u0/incoming/admin_hep-ph.paolonason.2268 which will then be moved to /u0/incoming/rejects

